The FIDS Theorems: Tensions between Multinode and Multicore Performance in Transactional Systems

Traditionally, distributed and parallel transactional systems have been studied in isolation, as they targeted different applications and experienced different bottlenecks. However, modern high-bandwidth networks have made the study of systems that are both distributed (i.e., employ multiple nodes) and parallel (i.e., employ multiple cores per node) necessary to truly make use of the available hardware. In this paper, we study the performance of these combined systems and show that there are inherent tradeoffs between a system's ability to have fast and robust distributed communication and its ability to scale to multiple cores. More precisely, we formalize the notions of a \emph{fast deciding} path of communication to commit transactions quickly in good executions, and \emph{seamless fault tolerance} that allows systems to remain robust to server failures. We then show that there is an inherent tension between these two natural distributed properties and well-known multicore scalability properties in transactional systems. Finally, we show positive results; it is possible to construct a parallel distributed transactional system if any one of the properties we study is removed.

==> sections/background.tex <==
\section{Background} \label{sec:background}

\newcolumntype{b}{X}
\newcolumntype{s}{>{\centering\arraybackslash\hsize=.5\hsize}X}
\newcolumntype{t}{>{\centering\arraybackslash\hsize=.25\hsize}X}

\begin{table}[t!]
  \centering
  \begin{tabularx}{\textwidth}{lbbbbbbb}
    \toprule
    \textbf{System} & \textbf{Sharded} & \textbf{Replicated} & \textbf{Shared-memory} & \textbf{DAP} & \textbf{IR} & \textbf{Fast-deciding} & \textbf{Seamless-FT} \\
    \midrule
    Spanner & Lock table
                & Read and Write Lock
                & N/A
                &
                & Yes \\
    TAPIR &
                       &
                       &
                       &
                       & Maybe \\
    Rolis &
                         &
                         &
                         &
                         & Maybe \\
    Janus &
                   &
                   &
                   &
                   & Yes \\
    Meerkat &
                   &
                   &
                   &
                   & Yes \\
    \bottomrule
  \end{tabularx}
  \caption{An overview of single-version, parallel, timestamp-based ordering schemes.}
  \label{tab:to_schemes}
\end{table}

==> sections/impossibility_single_shot.tex <==

\section{Impossibility results for single-shot transactions} \label{sec:impossibilities}

We start our analysis with assuming that all transactions are non-interactive, \emph{single-shot}~\cite{hstore07stonebreaker}. This simplifying assumption allows for fast protocols, where all transactions can be decomposed into groups of operations where each group can execute independently at a single shard. Since shards do not need to communicate to execute a transaction, one can easily imagine a protocol where the decision on whether to commit or abort can be learned in one round trip of communication between the client and the shards. Even with this simplification, we show that we cannot construct an algorithm that is simultaneously multicore and multishard scalable.

\subsection{Sharded Transactional Systems}

We now show that serializable sharded transactional systems cannot simultaneously achieve one-round-trip commitment, DAP, and strong invisible reads. That is, sharding while achieving these properties is impossible even if we do not tolerate any failures.
For that purpose, we begin with a lemma that characterizes the effect that the DAP and invisible reads properties together have on the ability of different transactions to be aware of each other during their execution.

\begin{lemma}\label{lem:inv-dap}
Let $S$ be a PDTS that provides both \DAP{} and invisible reads. Any transaction executed in $S$ whose write set is $W$ cannot cause any modifications on base objects accessed by transactions whose data set does not overlap with~$W$.
\end{lemma}

\begin{proof}
Consider a transaction $T$ with write set $W$, whose read set is empty (i.e. $W$ is equal to $T$'s data set). Then \DAP{} implies that $T$ cannot access any base object accessed by any transaction whose data set does not overlap $W$, as the lemma requires. Note that by the invisible reads property, any transaction $T'$ whose write set is also $W$ cannot execute any non-trivial primitives on base objects not accessed by $T$. Therefore, the lemma also holds for any such transaction $T'$. %\Naama{What is the difference between weak and strong DAP? Does the lemma hold for both?}
\end{proof}

We are now ready to prove the first main impossibility result. 

\begin{theorem}\label{thm:dist-impossibility}
There is no implementation of a PDTS that shards data across multiple nodes that simultaneously provides weak progress, serializability, invisible reads, one-round commitment, and disjoint-access parallelism.
\end{theorem}

\begin{proof}
Assume by contradiction that there exists an algorithm $A$ that implements a distributed transactional system with all of the properties in the theorem statement.

Consider a database with $2$ data items, $X_1, X_2$, partitioned on $2$ nodes. Consider two concurrent transactions, $T_1, T_2$, executed by two different clients. The read and write sets of the transactions are as follows: $R_{T_1} = \{X_1\}$, $W_{T_1} = \{X_2\}$, $R_{T_2} = \{X_2\}$, $W_{T_2} = \{X_1\}$. Consider the following executions.

\textsc{Solo Executions.} We define two executions, $S_1$, and $S_2$, corresponding to each of the two transactions $T_1$, and $T_2$ running in isolation, without the other one present in the execution. Let $m_{i,j}$\galy{This notation is never used} be the response client $C_i$ receives in the last round trip of transaction $T_i$ from node $j$. Note that since $A$ has single round trip termination and each execution $S_i$ has no conflicts, this last round trip must be the first one in which $C_i$ sent a non-trivial message to any node. Furthermore, by the correctness and weak progress properties of $A$, transaction $T_i$ successfully commits in $S_i$ and returns the initial value of $X_i$.

\textsc{Concurrent Execution.} We define an execution, $E_{concur}$, where $T_1$ and $T_2$ execute concurrently. Furthermore, on each node, each transaction is executed on different processes. Recall that this can happen since this is a parallel system, and the executing process for a transaction is arbitrarily chosen among the $n$ processes of each node.
Let both clients \galy{All references to clients should be to coordinators instead.} \galy{Why would a client necessarily send a non-trivial message? A coordinator might for instance send a message to a leader node and then only the latter one will send non-trivial messages. So maybe we should change it to be {\em the first non-trivial message associated with the tx}, and make sure that its round trip must still end at the coordinator.} (executing the two transactions) send their first non-trivial messages at the same time (i.e., both clients send their first non-trivial message before any node receives a non-trivial message from any client). Let the round trip in which client $C_i$ sends its first non-trivial message be $C_i$'s $r_i$th round trip.
Note that since no non-trivial messages have been sent so far in $E_{concur}$,
all messages associated with transaction $T_i$ so far must be the same as they were in the solo execution $S_i$. 
%the states of all processes and clients are the same as they were in their respective solo executions at the beginning of their last round trip. \Naama{Fix to match new definition. Something like: for each trivial message, if we remove it from the execution, all other messages have to be the same, so the state can't have changed...}

Note that when a client $C_i$ sends its first non-trivial message, it may concurrently send a message to each node. 
%However, since $A$ satisfies \DAP{}, a message to a node that does not contain one of $T_i$'s data items cannot result in a shared memory access.
%Therefore, such messages cannot affect other concurrent transactions on that node.
%
Now, let each node receive and service the message from the reading transaction before the message from the writing transaction in $E_{concur}$. More precisely, let $T_i$'s $r_i$ round-trip message to node $i$ arrive before $T_{i+1}$'s $r_{i+1}$ round-trip message, where addition is modulo 2.
Let each of the nodes complete its handler and send a reply to the first message before receiving the second message. Note that the reply to these messages must be the same as the reply sent in the corresponding solo execution, since all previous messages in the execution $E_{concur}$ that are associated with the other transaction have been trivial, and trivial messages do not affect the messages sent for other transactions. 
%Therefore, the executing processes must be in the same state as they were in the solo runs. ,

Furthermore, by Lemma~\ref{lem:inv-dap}, since $A$ satisfies \DAP{} and strong invisible reads, these first messages cannot cause shared memory to be modified on either of those nodes. Thus, the reply to the second message on each node must also be the same as the reply in the corresponding solo execution. Therefore, since the concurrent execution is indistinguishable to each client from its solo execution, both transactions commit in the concurrent execution, and return the initial value of both data items in their reads.

However, this means that there is a circular dependency between the two transactions; $T_2$ must occur before $T_1$, since it returns the initial value of $X_2$, before $T_1$ writes to it. Similarly, $T_1$ must occur before $T_2$, since it returns the initial value of $X_1$. This therefore contradicts serializability~\cite{bernstein86cc}. 
\end{proof}
\vspace{-1mm}

\subsection{Replicated Unsharded Systems}
So far, we've considered a PDTS in which node (or server) failures cannot be tolerated; if one of the nodes crashes, we lose all data items stored on that node, and cannot execute any transactions that access those data items.
%\Naama{Are we assuming each data item only has one node that stores it?}
However, in reality, server failures are common, and therefore many practical systems use replication to avoid system failures. Of course, the impossibility result of Theorem~\ref{thm:dist-impossibility} holds for a PDTS even for the more difficult case in which failures are possible and each node's data is replicated on several backups.

However, we now turn our attention to PDTS in which the entire database is stored on each node. This setting makes it plausible that a client could get away with accessing only one node to see the state of the data items of its transaction. However, we show that the impossibility of Theorem~\ref{thm:dist-impossibility} still holds for a system in which failures are tolerated without affecting transaction latency.

\begin{theorem}\label{thm:repl-impossibility}
There is no implementation of a PDTS that simultaneously provides weak progress, serializability, strong invisible reads, one-round commitment, $1$-seamless fault tolerance and disjoint-access parallelism.
\end{theorem}

The proof of this theorem is similar to the proof of Theorem~\ref{thm:dist-impossibility}. We build a cycle of dependencies between transactions where each neighboring pair in the cycle overlaps on a single data item that one of them reads and the other writes. The key is that because of the strong invisible reads, each read can happen before the write on the same data item without leaving a trace. However, to construct this cycle in the replicated case, we need at least 5 replicas and 5 transactions. This is because we can no longer separate the read and write of a single transaction on each node. 
The full proof is presented in Appendix~\ref{sec:impossibilityProof}.
%The proof is presented below.

%\input{sections/replicationProof}

==> sections/intro2.tex <==
\section{Introduction}

Transactional systems offer a clean abstraction for programmers to write concurrent code without worrying about synchronization issues. This has made them extremely popular and well studied in the last couple of decades. There are two classes of transactional systems that have mostly been treated separately in the literature: %However, the theoretical literature on transactional systems has studied
\emph{parallel transactional systems} and \emph{distributed transactional systems}. %mostly in isolation.

Parallel transactional systems (PTS), such as software transactional memory systems~\cite{attiya2011inherent} and single-node parallel databases~\cite{tu13silo}, generally assume a model where an application is running on a single node with multiple processes sharing the same memory. These systems are designed to take advantage of multicore architectures and support applications that require high processing power. Therefore, their primary concern for performance is achieving \emph{multicore scalability}, i.e., adding cores to the system should linearly increase performance.

In contrast,
distributed transactional systems (DTS), like distributed key-value stores and distributed databases~\cite{bernstein86cc}, generally assume a model with multiple single-process nodes connected through a network. These systems are designed to support applications that emphasize big data and high load way beyond the capacity of a single node, or require high availability, or both. Therefore, their main concern is to provide efficient \emph{sharding} (i.e. distributing data across multiple nodes) and \emph{replication} (i.e. creating copies of the data on multiple nodes) mechanisms to go along with the transaction processing protocols.
%to provide \emph{low latency} and \emph{high availability}. %Sharding means distributing the data across multiple nodes, and thus, mechanisms to support distributed transactions are required, while replication creates copies of the data on multiple nodes, and thus mechanisms to consistently process transactions on multiple copies of the data are required.


In this paper, we consider \emph{parallel distributed transactional systems} (PDTS), that combine both types of systems above. That is, we ask what can be done if the nodes in a sharded or replicated transactional system have multiple cores; can we achieve high availability, low latency \emph{and} multicore scalability in a single system?
This question is motivated by the needs of real systems. As was demonstrated by recent work by Szekeres et al. in a system called Meerkat~\cite{szekeres2020meerkat}, combining insights from both the distributed and the parallel transactional literatures is non-trivial, but highly beneficial. 
%Szekeres et al. presented Meerkat, a PDTS that leverages the multicore nature of machines in a distributed system for better performance.
\Naama{Maybe we can expand a bit here, to emphasize why PDTS is important in practice.}

We study PDTS from a theoretical point of view. We present the first model that combines distributed and parallel transactions, and consider desirable system properties drawn from both literatures. In particular, we show that it is impossible to design a PDTS that simultaneously achieves \emph{disjoint access parallelism}, \emph{strong invisible readers}, \emph{one round-trip commitment}, and \emph{seamless fault tolerance} while maintaining a basic notion of progress and safety in the form of serializability. On the positive side, we show that any subset of these properties \emph{is} achievable.
%that are known to be desirable for high availability, scalability, and low latency.

Disjoint access parallelism and invisible readers are properties commonly considered in the parallel transactional systems literature. They have been extensively studied in both theory and practice~\cite{attiya2011inherent,szekeres2020meerkat,peluso2015disjoint,attiya2015disjoint,tu2013speedy}, and are known to increase multicore scalability. Intuitively, disjoint access parallelism prevents processes from contending on shared memory if they execute transactions that do not conflict. The invisible readers property ensures that reading transactions do not modify shared memory. This helps avoid cache coherence misses that cause poor scalability in practice.
Interestingly, in this paper we observe that there is a gap between the notion of invisible reads used in the theory literature and the notion used in the systems literature. At a high level, theoretical definitions of invisible reads constrain only read-only transactions, whereas many systems that aim for invisible readers avoid causing any shared memory modifications due to read operations in any transaction~\cite{tu2013speedy,szekeres2020meerkat}. We formalize this difference, and define \emph{strong invisible reads} to capture the stricter notion from the systems literature.

One round-trip commitment and seamless fault tolerance are notions drawn from the distributed transactional systems literature. These systems often have a \emph{client} that sits on a physically different machine than the servers that run the transaction. Latency and high availability are measured from the point of view of the client. Often, transactional systems are designed so that a transaction coordinator (either the client itself or some designated server process) optimistically sends read requests to the servers to try to locally execute its transaction, and then \emph{validates} its local execution with the servers. 
The one round-trip commitment property intuitively requires that the transaction coordinator can execute its validation within one network round trip, to quickly learn whether the transaction committed or aborted. 
Seamless fault-tolerance intuitively allows the system to \emph{seamlessly} tolerate failures, i.e., no performance degradation is sensed on server failure by the clients. Both of these properties have been shown to have a crucial role in creating efficient and highly available systems; recent works in this space~\cite{zhang18tapir, mu16janus, kraska13mdcc} significantly improve on the state-of-the-art by enforcing these properties. However, these properties have not been formalized, and have instead only been used intuitively to describe some system behavior. In this paper we provide the first formal definitions of both of these notions in the transactional system context.

%The preferred correctness property among all transactional systems (whether distributed or parallel) is \emph{serializability} which requires transactions to appear as if they executed serially, one after the other~\cite{papadimitriou1979serializability}. Furthermore, these systems are expected to at least provide \emph{weak progress} guarantees, which require that transactions that do not encounter conflicts or more failures than the system tolerates to terminate successfully, i.e., to commit. This is a basic requirement that prevents trivial solutions.

Thus, our results show inherent limitations in the merging of parallel and distributed transactional systems; it is impossible to have it all. On the other hand, we show that giving up any one of these desirable properties does admit feasible solutions. Furthermore, some of these properties only need to be slightly relaxed, rather than completely discarded, to allow system implementation. For example, we show that it is possible to build a PDTS that ensures disjoint access parallelism, one round-trip commitment, seamless fault tolerance, and \emph{weak} invisible reads, where only read-only transactions are invisible. Similarly, a system that tolerates failures, but with slightly increased latency, can also achieve the other three properties. We believe that this work motivates further study of PDTS, both from a theoretical and practical lens.

In summary, the contributions of this paper are as follows:

\begin{itemize}
    \item We provide the first formal model capturing PDTS
    \item We formally define \emph{strong invisible reads}, \emph{one round-trip commitment}, and \emph{seamless fault tolerance}, three notions that are well known in the transactional systems literature that have so far been used informally
    \item We show that it is impossible to achieve all of these properties and disjoint access parallelism in a PDTS that is serializable and has minimal progress; this result holds for both replicated and sharded systems, even if the sharded systems do not tolerate failures

    \item Finally, we show that it \emph{is} possible to construct a PDTS that is serializable with weak progress, and guarantees any subset of the above properties.
\end{itemize}


==> sections/old-intro-spaa.tex <==


Transactional systems can be roughly divided into two classes: %However, the theoretical literature on transactional systems has studied
\emph{parallel transactional systems (PTS)}, which are designed to run on a single multicore node, and \emph{distributed transactional systems (DTS)}, which are designed to run on multiple nodes, but generally assume each node only has one core. %mostly in isolation.

%Parallel transactional systems (PTS), such as software transactional memory systems~\cite{attiya2011inherent} and single-node parallel databases~\cite{tu13silo}, generally assume a model where an application is running on a single node with multiple processes sharing the same memory. These systems are designed to take advantage of multicore architectures and support applications that require high processing power. Therefore, their primary concern for performance is achieving \emph{multicore scalability}, i.e., adding cores to the system should linearly increase performance.

%In contrast, distributed transactional systems (DTS), like distributed key-value stores and distributed databases~\cite{bernstein86cc}, generally assume a model with multiple single-process nodes connected through a network. These systems are designed to support applications that emphasize big data and high load way beyond the capacity of a single node, or require high availability, or both. Therefore, their main concern is to provide efficient \emph{sharding} (i.e. distributing data across multiple nodes) and \emph{replication} (i.e. creating copies of the data on multiple nodes) mechanisms to go along with the transaction processing protocols.
%%to provide \emph{low latency} and \emph{high availability}. %Sharding means distributing the data across multiple nodes, and thus, mechanisms to support distributed transactions are required, while replication creates copies of the data on multiple nodes, and thus mechanisms to consistently process transactions on multiple copies of the data are required.

Traditionally, PTS and DTS have been studied separately in the literature, due to the different nature of the applications they target. In particular, since network communication was, for many years, much slower than local computation, applications that require multiple nodes could not gain any significant benefit from optimizing parallelism within each node. Thus, practical considerations for single-node vs multi-node applications led their study to be almost entirely separate. Due to these different settings, the design goals of PTS and DTS also differ; while PTS design is primarily concerned with increasing \emph{mulitcore scalability}, DTS design is focused on providing efficient \emph{sharding} and \emph{replication} to provide low latency and high availability.


%Motivated by recent increase in network performance, in this paper we consider \emph{parallel distributed transactional systems} (PDTS), that combine both types of systems above. That is, we ask what can be done if the nodes in a sharded or replicated transactional system have multiple cores; can we achieve high availability, low latency \emph{and} multicore scalability in a single system?
%This question is motivated by the needs of real systems. 
Due to increased bandwidth on modern networks, distributed systems are no longer solely bottlenecked by the network. In particular, while network latency is still significant compared to computations within a single node, sequential processing within each node is no longer enough to handle the throughput that a network can deliver. Thus, to keep up with the capabilities of modern hardware, transactional systems must be designed while optimizing \emph{both} network communication \emph{and} multicore scalability. As was demonstrated by recent work by Szekeres et al. in a system called Meerkat~\cite{szekeres2020meerkat}, combining insights from both the distributed and the parallel transactional literatures is non-trivial, but highly beneficial. 
\Naama{Cite others like Rolis and whatever Rolis cites for this? Could be nice to present this as an active new direction in the systems community, say we are the first to consider theoretical aspect.}
%Szekeres et al. presented Meerkat, a PDTS that leverages the multicore nature of machines in a distributed system for better performance.
%\Naama{Maybe we can expand a bit here, to emphasize why PDTS is important in practice.}

Thus, in this paper we consider \emph{parallel distributed transactional systems} (PDTS), that combine both types of systems above. That is, we ask what can be done if the nodes in a sharded or replicated transactional system have multiple cores; can we achieve high availability, low latency \emph{and} multicore scalability in a single system?

\aaasz{TODO: strong invisible readers has been formally specified}
We study PDTS from a theoretical point of view. We present the first model that combines distributed and parallel transactions, and consider desirable system properties drawn from both literatures. We observe that some properties that are often considered the gold standard for parallel or distributed transactional systems have in fact never been formally defined. In particular, we consider two properties drawn from each literature: \emph{disjoint access parallelism (DAP)} and \emph{invisible readers} from the parallel transactional literature, and \emph{one round-trip commitment} and \emph{seamless fault tolerance} from the distributed one. Our contribution is two-fold. 
First, we formalize these properties in the context of PDTS. Of the four properties above, we observe that only DAP has been formalized. We find that this is not a coincidence; while all of them are easy to understand intuitively, it is non-trivial to formalize their meaning without artificially restricting solutions that achieve them. Our first contribution is therefore to formalize the properties of \emph{invisible readers}, \emph{one round-trip commitment}, and \emph{seamless fault tolerance}.
 
We then study systems that achieve all four of the above properties. We show that it is impossible to have a \emph{serializable} PDTS with minimal progress that simultaneously achieves all four of these properties. On the other hand, we show that relaxing any of these properties does lead to feasible systems. 
%In particular, we show that it is impossible to design a PDTS that simultaneously achieves \emph{disjoint access parallelism}, \emph{strong invisible readers}, \emph{one round-trip commitment}, and \emph{seamless fault tolerance} while maintaining a basic notion of progress and safety in the form of serializability. On the positive side, we show that any subset of these properties \emph{is} achievable.
%that are known to be desirable for high availability, scalability, and low latency.

Disjoint access parallelism and invisible readers 
%are properties commonly considered in the parallel transactional systems literature. They 
have been extensively studied in both theory and practice~\cite{attiya2011inherent,szekeres2020meerkat,peluso2015disjoint,attiya2015disjoint,tu2013speedy}, and are known to increase multicore scalability. Intuitively, disjoint access parallelism prevents processes from contending on shared memory if they execute transactions that do not conflict. The invisible readers property ensures that reading transactions do not modify shared memory. This helps avoid cache coherence misses that cause poor scalability in practice.
Interestingly, in this paper we observe that there is a gap between the notion of invisible reads used in the theory literature and the notion used in the systems literature. At a high level, theoretical definitions of invisible reads constrain only read-only transactions, whereas many systems that aim for invisible readers avoid causing any shared memory modifications due to read operations in any transaction~\cite{tu2013speedy,szekeres2020meerkat}. We formalize this difference, and define \emph{invisible reads} to capture the stricter notion from the systems literature.

One round-trip commitment and seamless fault tolerance are notions drawn from the distributed transactional systems literature. These systems often have a \emph{client} that sits on a physically different machine than the servers that run the transaction. Latency and high availability are measured from the point of view of the client. Often, transactional systems are designed so that a transaction coordinator (either the client itself or some designated server process) optimistically sends read requests to the servers to try to locally execute its transaction, and then \emph{validates} its local execution with the servers. 
The one round-trip commitment property intuitively requires that the transaction coordinator can execute its validation within one network round trip, to quickly learn whether the transaction committed or aborted. 
Seamless fault tolerance intuitively allows the system to \emph{seamlessly} tolerate failures, i.e., no performance degradation is sensed on server failure by the clients. Both of these properties have been shown to have a crucial role in creating efficient and highly available systems; recent works in this space~\cite{zhang18tapir, mu16janus, kraska13mdcc} significantly improve on the state-of-the-art by enforcing these properties. However, these properties have not been formalized, and have instead only been used intuitively to describe some system behavior. In this paper we provide the first formal definitions of both of these notions in the transactional system context.

%The preferred correctness property among all transactional systems (whether distributed or parallel) is \emph{serializability} which requires transactions to appear as if they executed serially, one after the other~\cite{papadimitriou1979serializability}. Furthermore, these systems are expected to at least provide \emph{weak progress} guarantees, which require that transactions that do not encounter conflicts or more failures than the system tolerates to terminate successfully, i.e., to commit. This is a basic requirement that prevents trivial solutions.

Thus, our results show inherent limitations in the merging of parallel and distributed transactional systems; it is impossible to have it all. On the other hand, we show that giving up any one of these desirable properties does admit feasible solutions. Furthermore, some of these properties only need to be slightly relaxed, rather than completely discarded, to allow system implementation. For example, we show that it is possible to build a PDTS that ensures disjoint access parallelism, one round-trip commitment, seamless fault tolerance, and \emph{weak} invisible reads, where only read-only transactions are invisible. Similarly, a system that tolerates failures, but with slightly increased latency, can also achieve the other three properties. We believe that this work motivates further study of PDTS, both from a theoretical and practical lens.

In summary, the contributions of this paper are as follows:

\begin{itemize}
    \item We provide the first formal model capturing PDTS
    \item We formally define \emph{invisible reads}, \emph{fast deciding}, and \emph{seamless fault tolerance}, three notions that are well known in the transactional systems literature that have so far been used informally
    \item \aaasz{TODO: we are the first to show a tension between properties specific to DTSes and properties specific to PTSes} We show that it is impossible to achieve all of these properties and disjoint access parallelism in a PDTS that is serializable and has minimal progress; this result holds for both replicated and sharded systems, even if the sharded systems do not tolerate failures

    \item Finally, we show that it \emph{is} possible to construct a PDTS that is serializable with weak progress, and guarantees any subset of the above properties.
\end{itemize}


==> sections/old-intro.tex <==
\section{Introduction}

Transactional systems offer a clean abstraction for programmers to write concurrent code without worrying about synchronization issues. This has made them extremely popular and well studied in the last decades. There are two classes of transactional systems that have mostly been treated separately in the literature; %However, the theoretical literature on transactional systems has studied
\emph{parallel transactional systems} and \emph{distributed transactional systems}. %mostly in isolation.

Parallel transactional systems (PTS), such as software transactional memory systems~\cite{attiya2011inherent} and single-node parallel databases~\cite{tu13silo}, generally assume a model where an application is running on a single node with multiple processes sharing the same memory. These systems are designed to take advantage of multicore architectures and support applications that require high processing power. Therefore, their primary concern is achieving \emph{multicore scalability}, i.e., adding cores to the system should linearly increase performance. \emph{Disjoint-access parallelism} and \emph{invisible readers} are two properties that have been proposed and long studied in the literature that are known to increase multicore scalability. Intuitively, the two properties prevent processes from contending on shared memory if they execute transactions that do not conflict. \aaasz{TODO: more detail} This guarantees multicore scalability when the system executes non-conflicting transactions.

Distributed transactional systems (DTS), like distributed key-value stores and distributed databases~\cite{bernstein86cc}, generally assume a model with multiple single-process nodes connected through a network. These systems are designed to support applications that emphasize big data and high load way beyond the capacity of a single node, or require high availability, or both. Therefore, their main concern is to provide efficient \emph{sharding} and \emph{replication} mechanisms to go along with the transaction processing protocols. Sharding means distributing the data across multiple nodes, and thus, mechanisms to support distributed transactions are required, while replication creates copies of the data on multiple nodes, and thus mechanisms to consistently process transactions on multiple copies of the data are required. Many of the existing distributed transactional systems use two-phase commit, to deal with sharding, and state machine replication, for consistent replication, two mechanisms heavily studied in the literature. Recent works in this space~\cite{zhang18tapir, mu16janus, kraska13mdcc} improve on the state-of-the-art by proposing replication mechanisms that allow better availability and latency through \emph{one round-trip commitment} and \emph{seamless fault-tolerance}. The one round-trip commitment property intuitively requires that the transaction coordinator (which is either the client itself or some other process that initialized the execution of the transaction) learns after one round-trip, after the execution phase, the outcome of the transaction. Seamless fault-tolerance intuitively allows the system to \emph{seamlessly} tolerate failures, i.e., no performance degradation is sensed on failure by the clients.

The preferred correctness property among all transactional systems is \emph{serializability} which requires transactions to appear as if they executed serially, one after the other. Furthermore, these systems are expected to at least provide \emph{weak progress} guarantees, which require that transactions that do not encounter conflicts or more failures than the system tolerates to terminate successfully, i.e., to commit.

Recently, Meerkat~\cite{szekeres2020meerkat} proposes a \emph{parallel distributed transactional system} (PDTS), in which the multicore nature of each machine in the distributed system is leveraged for better performance. The system provides serializability and weak progress, together with the two properties introduced by the recent distributed transactional systems, i.e., one round-trip commitment and seamless fault-tolerance, and one of the properties introduced by the parallel transactional systems, disjoint-access parallelism. It does not, however, provide any of the invisible reads properties. This paper is the first to consider PDTS from a theoretical lens. We model this setting, outline the desirable properties for such systems that draw from both literature on PTS and literature on DTS. We present an impossibility theorem showing that no PDTS can provide all these properties simultaneously \aaasz{TODO: more detail}. However, we show that for every subset of these properties, it is possible to construct a PDTS that guarantees them.

In summary, the paper makes the following contributions:

\begin{itemize}
    \item it is the first to formalize a model to study PDTS and several desirable properties for these systems
    \item it shows that: 
        \begin{itemize}
            \item no PDTS that shards data on multiple nodes can simultaneously achieve all 3 properties and provide serializability and weak progress
            \item no PDTS that replicates data on multiple nodes (and optionally also shards data on multiple nodes) can simultaneously achieve all 4 properties and provide serializability and weak progress
        \end{itemize}
    \item it shows that it is possible to construct a PDTS for every case where we sacrifice any of the properties and provide the others
\end{itemize}

%\begin{itemize}
%    \item Transactional systems have been extremely well studied since the 70s. This is natural, since they can provide a clean abstraction for programmers to write concurrent code without worrying about synchronization issues.
%    \item Generally, the transactional systems literature has focused on the multicore shared memory setting.
%    \item \Naama{Not sure how to work this in... feels like to contradicts the claim that transactional systems are generally made for concurrent shared memory} database theory does not model multicores (they assume executions can be modeled as sequentially consistent transactional operations)
%    \item However, recent applications that emphasize big data, high load, and require high  availability  have led to work on \emph{distributed transactions}; transactional systems that reside not only on one multicore machine, but are distributed over several machines.
%    \item Something about how most literature uses traditional distributed techniques, like state machine replication
%    \item Recently, Meerkat and others consider \emph{concurrent distributed transactions} (or another term), in which the multicore nature of each machine in the distributed system is leveraged for higher scalability/lower latency/higher throughput etc etc
%    \item This paper is the first to consider parallel distributed transactions from a theoretical lens. We model this setting, outline desirable properties for such systems that draw from both shared memory transactions literature and distributed literature. We present an impossibility theorem showing that no system can provide all these properties simultaneously.
%    \item However, we show that for every subset of these properties, it is possible to construct a concurrent distributed transactional system that guarantees all of the subset.
%\end{itemize}

==> sections/old-proof-pieces.tex <==


%Before delving into the proof of the theorem, we first make a useful observation about how long it must take in a sharded system for some process to learn a transaction's read values. This will help in the theorem proof relate the potential depth of a fast-deciding execution to the depth at which transactions know their write set.

%\begin{observation}\label{obs:sharded-learning}
%Consider any transaction $T$ whose read set spans multiple shards.
%There is no execution $E$ of any PDTS implementation $I$ in which $T$ commits and there exists a prefix $P$ of $E$ such that $d_E(T,P)<2$ and some process knows the decided value of all of the data items in $T$'s read set in $P$.
%\end{observation}

%\begin{proof}
%    This observation can be seen by recalling the setup of PDTS systems and the corresponding relevant definitions. Recall that the initiating client in a PDTS does not have access to any of the data, and that in sharded systems, no process on a node $N$ knows the value of any data item not on $N$ outside the execution of a \handler{} on behalf of some transaction. Therefore, at least one message must be sent by the initiating client for $T$, and at least one more message after that must be sent from inside corresponding handler on each of the nodes that contain items from $T$'s read set to some aggregating process. Note that if no such aggregating process exists, then for every process in the system, we could construct an execution indistinguishable to that process in which a value on a different node has been changed, and therefore no single process would have knowledge of the decided values for $T$. 
%   By the definition of the depth of steps, the initial message from the client plus the aggregating message mean that knowledge of all of $T$'s decided values occurs at a depth of at least 2.
%\end{proof}


\begin{proof}
Assume by contradiction that there exists an implementation $I$ of a PDTS with all the properties in the theorem statement.

Consider a database with $3$ data items, $X_1, X_2, X_3$, partitioned on $3$ nodes, $N_1,N_2, N_3$ respectively. Consider two transactions, $T_1, T_2$, with the following data sets: $T_1$'s read set is $X_1$ and $X_2$, both decided initially. Its write set is $X_3$ if its reads both return the initial values of $X_1$ and $X_2$, in which case it writes a value different from $X_3$'s initial value. Its write set is empty otherwise. For $T_2$, its read set is $X_2$ and $X_3$, decided initially, and its write set is $X_1$ if both reads return the initial values of their data items and empty otherwise. If its write set is non-empty, it writes a value different from $X_1$'s initial value. Let $T_1$ be executed by a client $C_1$ and $T_2$ be executed by a different client $C_2$.

Consider the following executions.
%In each of them that includes $T_i$ or $T_{iW}$, $C_i$ runs the \coordhandler{} of $T_i$ or $T_{iW}$. 

\textsc{Solo Executions.} We define two executions $S_1,S_2$, corresponding to $T_1,T_2$ respectively running in isolation, without the other transaction present in the execution. Both executions are synchronous and failure-free. 

\textit{Claim: Since $I$ is fast-deciding and each execution $S_i$ is synchronous and has no failures or transaction conflicts, both transactions must have a depth of at most 4 in their respective executions.}

To see this, note that by the definition of fast-deciding, if the depth of transaction $T_i$ in $S_i$ has depth at least 3, the empty prefix of $S_i$ must have a continuation $C_i$ of partial depth $d_{S_i}(T_i, C_i) \leq 2$ in which the values of both data items in the read sets are known by some process to be decided, and therefore the write set is known by that process to be decided as well. By~\cref{cor:fast-deciding}, the depth of $T_i$ in $S_i$ must be at most 2 more than the depth of $C_i$, and therefore is at most 4.

Note that by weak progress, $T_i$ commits in $S_i$ and by serializability, $T_i$ returns the initial values of its read set and therefore modifies its write set.


\textsc{Concurrent Execution.} We define an execution, $E_{concur}$, where $T_1$ and $T_2$ execute concurrently. On each node, each transaction is executed on different processes. Recall that this can happen since this is a parallel system, and the executing processes for a transaction are arbitrarily chosen among the idle processes of each node.
In $E_{concur}$, we let both transactions run until, for each transaction $T_i$, some process $p_i$ knows the decided write set of $T_i$.
We then let the next messages for each transaction be sent in $E_{concur}$, and let any message sent at this point by a handler for $T_1$ reach $N_1$ and $N_2$ before any message sent at this point by a handler of $T_2$ to these nodes. However, for node $N_3$, we let the reverse happen; messages sent by handlers of $T_2$ at this point reach it before messages sent on behalf of $T_1$ to $N_3$. Furthermore, we let each message handler at this point run to completion before the node receives the next message. Finally, we let the rest of the handlers of $T_1$ and $T_2$ run to completion.

We now claim that execution $E_{concur}$ is indistinguishable to processes running $T_i$ from $S_i$. To do so, we consider the execution in two phases; the phase before the two transactions achieve knowledge of their data sets, and the phase afterwards.

\textsc{Phase 1 of $E_{concur}$.}
Note that by~\cref{obs:sharded-learning}, no process learns the decided values of $T_i$'s read set, and therefore the decided write set, until at least depth $2$. Therefore, the partial depth of each transaction in $E_{concur}$ is at least 2 by the end of phase 1.

\textit{Claim: In $E_{concur}$, there is no prefix $P_i$ of partial depth $d_{E_{concur}}(T_i, P_i) \leq 2$ in which $T_i$ makes any visible modifications to shared memory.}

Assume by contradiction that the claim does not hold. Note that for any prefix $P$ of $E_{concur}$ in which $T_i$'s read set's values are not decided, $T_i$'s decided write set in $P$ is empty. Therefore, by~\cref{lem:future-writes}, in any such prefix $T_i$ may not make any modifications to shared memory objects accessed by \emph{any} transaction. Furthermore, by~\cref{obs:sharded-learning}, no process \emph{knows} the write set of $T_i$ in any prefix of depth less than $2$.
\end{proof}

\begin{proof}
Assume by contradiction that there exists an implementation $I$ of a PDTS with all the properties in the theorem statement.

Consider a database with $2$ data items, $X_1, X_2$, partitioned on $2$ nodes, $N_1,N_2$ respectively. Consider four transactions, $T_1, T_2,T_{1W},T_{2W}$.
The read and write sets of the transactions are as follows: 
%$W_{T_1} = \{X_1\}$, $R_{T_1} = \{X_2\}$, $W_{T_2} = \{X_2\}$, $R_{T_2} = \{X_1\}$, 

\begin{center}
\begin{tabular}{ |P{0.4cm}||P{0.7cm}|P{0.7cm}|P{0.7cm}|P{0.7cm}|  }
 \hline
 \multicolumn{5}{|c|}{Transactions write and read sets} \\
 \hline
 $T$ & $T_1$ & $T_{1W}$ & $T_{2W}$ & $T_2$ \\
 \hline
 $W_T$ & $X_1$ & $X_1$ & $X_2$ & $X_2$ \\
 $R_T$ & $X_2$ & $\phi$ & $\phi$ & $X_1$ \\
 \hline
\end{tabular}
\end{center}

Consider two clients, $C_1,C_2$. 
Consider the following synchronous executions.
In each of them that includes $T_i$ or $T_{iW}$, $C_i$ runs the \coordhandler{} of $T_i$ or $T_{iW}$. 

\textsc{Solo Executions.} We define four executions, $S_1,S_2,S_{1W},S_{2W}$, corresponding to $T_1,T_2,T_{1W}$ or $T_{2W}$ respectively running in isolation, without the other transactions present in the execution. Note that since $I$ has single round trip termination and each execution $S_i$ is synchronous and has no node crashes or transaction conflicts, the last round trip of transaction $T_i$ in $S_i$ must be the first one in which a non-trivial message is sent on behalf of $T_i$ to any node. Furthermore, by the weak progress property of $I$, transaction $T_i$ commits in $S_i$ and returns the initial value of $X_{(i\text{ mod }2)+1}$.

\textsc{Concurrent Execution.} We define an execution, $E_{concur}$, where $T_1$ and $T_2$ execute concurrently. On each node, each transaction is executed on different processes. Recall that this can happen since this is a parallel system, and the executing processes for a transaction are arbitrarily chosen among the idle processes of each node.
Let the first non-trivial message associated with each of the transactions be sent at the same time (i.e., ****** both clients send their first non-trivial message before any node receives a non-trivial message from any client). Let the round trip in which client $C_i$ sends its first non-trivial message be $C_i$'s $r_i$th round trip.
Note that since no non-trivial messages have been sent so far in $E_{concur}$,
all messages associated with transaction $T_i$ so far must be the same as they were in the solo execution $S_i$. 
%the states of all processes and clients are the same as they were in their respective solo executions at the beginning of their last round trip. \Naama{Fix to match new definition. Something like: for each trivial message, if we remove it from the execution, all other messages have to be the same, so the state can't have changed...}

Note that when a client $C_i$ sends its first non-trivial message, it may concurrently send a message to each node. 
%However, since $I$ satisfies \DAP{}, a message to a node that does not contain one of $T_i$'s data items cannot result in a shared memory access.
%Therefore, such messages cannot affect other concurrent transactions on that node.
%
Now, let each node receive and handle the message from the reading transaction before the message from the writing transaction in $E_{concur}$. More precisely, let $T_1$'s $r_1$th round-trip message to the node with $X_1$ arrive before $T_2$'s $r_2$th round-trip message; and $T_2$'s $r_2$th round-trip message to the node with $X_2$ arrive before $T_1$'s $r_1$th round-trip message.
Let each of the nodes complete its handler and send a reply to the first message before receiving the second message. Note that the reply to these messages must be the same as the reply sent in the corresponding solo execution, since all previous messages in the execution $E_{concur}$ that are associated with the other transaction have been trivial, and trivial messages do not affect the messages sent for other transactions. 
%Therefore, the executing processes must be in the same state as they were in the solo runs. ,

Furthermore, by Lemma~\ref{lem:inv-dap}\galy{How does this follow from the lemma? Here the write set of each transaction does overlap with the data set of the other transaction. I don't understand how sharding affects the impossibility result and how we may prove impossibility without 1-seamless fault tolerance (which allows us to compare the concurrent executions with executions in which a node fails but the transaction must still decide in 1RT).}, since $I$ satisfies \DAP{} and strong invisible reads, these first messages cannot cause shared memory to be modified on either of those nodes. Thus, the reply to the second message on each node must also be the same as the reply in the corresponding solo execution. Therefore, since the concurrent execution is indistinguishable to each client from its solo execution, both transactions commit in the concurrent execution, and return the initial value of both data items in their reads.

However, this means that there is a circular dependency between the two transactions; $T_2$ must occur before $T_1$, since it returns the initial value of $X_2$, before $T_1$ writes to it. Similarly, $T_1$ must occur before $T_2$, since it returns the initial value of $X_1$. This therefore contradicts serializability~\cite{bernstein86cc}. \aaasz{TODO: I believe here we need to assume the writes the two transactions perform are distinct than the initial values (for our definition of serializability to apply)}
\end{proof}
\vspace{-1mm}



\begin{lemma}\label{lem:future-writes}
Let $I$ be an implementation of a PDTS that provides both \DAP{} and invisible reads, let $T$ be a transaction in an execution $E$ of $I$, and let $W$ be $T$'s known decided write set in $E$. Then $T$ cannot cause any modifications \Naama{visible to any concurrent transaction} 
%on base objects that are accessed in $E$ by any transaction 
$T'$ whose known decided read and write sets in $E$ do not overlap with $W$.
\end{lemma}

\begin{proof}
Let $I$ be an implementation of a PDTS that satisfies \DAP{} and invisible reads.
Assume by contradiction that there is some execution $E$ of $I$ in which a transaction $T$'s known decided write set is $W$ but which causes modifications visible to 
%on base objects accessed by 
a concurrent transaction $T'$ whose known decided read and write sets do not overlap with $W$ in $E$. Let $D$ be the union of $T'$'s known decided read and write sets in $E$. 
Let $p$ be a process that runs a handler associated with $T$ which modifies a base object accessed by $T'$.
Since no data item $d \in D$ is known to be decided to be in $T$'s write set in $E$, for every process $q$ there must be an execution of $I$, indistinguishable to $q$ from $E$, in which no data item $d \in D$ is decided to be in $T$'s write set. Let $E'$ be such an execution indistinguishable to $p$ from $E$.
Similarly, there is an execution $E''$ indistinguishable to $p$ from $E'$, in which no data item $d \notin D$ is decided to be in $T'$'s read or write sets.
Since no data item $d \in D$ is decided to be in $T$'s write set in $E''$ \Naama{not sure this is true}, and no data item $d \notin D$ is decided to be in $T'$'s read or write sets in $E''$, 
there must be an \continuation{} of $E''$ in which no data item $d \in D$ is in $T$'s final write set and no data item $d \notin D$ is in $T'$'s final read or write sets.\galy{This is not necessarily the case for the transaction program of $T$, but rather -- there exists another transaction program that starts the same and then does not write to any additional data item. We face here the problem of abusing the transaction notation $T$, which sometimes refers to a specific transaction program and sometimes refers to the transaction as its steps in the execution---which may match multiple transaction programs. But saying here that there exists such an extension in which $T$ and $T'$ are replaced with other transactions will be confusing.} Then such an \continuation{} of $E''$ is an execution of $I$ that violates~\Cref{lem:inv-dap}.
\end{proof}


==> sections/old-pseudocode.tex <==

\begin{figure}
\begin{lstlisting}
Shared Memory:
    DataItem:
        lock
        seqNum
        value
    DataItem* dataItems[]
       
Process code:
    Upon receiving execution phase message for data item d from C:
        while d is locked{}
        send (d.val, d.seqNum) to C
    Upon receiving verification phase message M for T from C:
        bool success = true
        for each data item d in T:
            if d is locked or d.seqNum != seqNum of d in M:
                send abort to C
                success = false
                break
            if T is not read-only:
                if not tryLock(d.lock):
                    send abort to C
                    success = false
                    break
        if success:
            send commit to C
    Upon receiving commit message for T from C:
        for each data item d in T.W:
            write new value of d on d.value
        for each data item d in T.D:
            unlock(d.lock)
    Upon receiving abort message for T from C:
        for each data item d in T.D:
            unlock(d.lock)
\end{lstlisting}
\caption{Pseudocode for transactional system that sacrifices strong invisible reads.}
\label{alg:noInvReads}
\end{figure}

==> sections/properties-old.tex <==
\section{Desirable properties}

In this section we describe in detail a few properties that are valuable for distributed and parallel transactional storage systems -- they promise high availability, scalability, and performance.

To provide transactions, PDTSes use a parallel and distributed \emph{concurrency control protocol}. Non-deterministic, parallel, and distributed concurrency control protocols roughly follow the template protocol in \autoref{alg:coord_template} and \autoref{alg:proc_template}. Transaction processing is
orchestrated by a \emph{coordinator} process (which runs either at a client or at a server machine). It begins with an \emph{execution phase} where the coordinator receives read and write requests from the client and processes them using the \textbf{read} and \textbf{write} procedures. The procedures are either local (e.g., the key is already in the readSet or writeSet) or remote (e.g., data needs to be fetched from a server). The coordinator collects the \emph{readSet} and \emph{writeSet} of the transaction and then starts the \emph{commitment phase}. This phase involves an atomic commitment protocol (such as two-phase commit) to ensure that the transaction is atomic -- it either executes at all nodes its data sets spans or at none of them. The \textbf{prepare} procedure may involve a multiple round-trip communication, and it's role is to ensure all nodes the transaction spans are ready to commit the transaction. They manifest this through \emph{votes} and if \emph{all} votes of the respective nodes are to commit the transaction, then the coordinator calls the \emph{commit} procedure, otherwise it calls the \emph{abort} procedure.

When any of the coordinator procedures is remote, a \emph{participant} process (which runs on a server machine) receiving the procedure call, invokes a \textbf{handler}. We 

\Naama{broken sentence.}


which sometimes utilizes memory synchronization primitives,
like locks, CASes, etc., which we emphasized through the \textbf{synchronize} procedure, a function of the data in the message received. These synchronization primitives protect access to either shared data or metadata utilized by the concurrency control protocol.


\definecolor{comment-color}{rgb}{0.6627, 0.7176, 0.7764}

\lstdefinestyle{lststyle}
{
    language = python,
    basicstyle=\footnotesize\ttfamily,
    keywordstyle = {\color{blue}\bfseries},
    morecomment=[l][\color{comment-color}]{//},
}

\renewcommand{\figurename}{Algorithm}

\begin{figure}[t!]
\begin{lstlisting}[style=lststyle, frame=tlrb, escapechar=@]
//Execution phase
readSet = {}; writeSet = {};
for each key R the client reads:
    result = @\textbf{read}@(R);
    Add pair <R, result> to readSet;
    
for each key W, value v the client writes:
    @\textbf{write}@(W, v);
    Add pair <W, v> to writeSet;

//Prepare phase
Create transaction message T containing the readSet and writeSet;

@\textbf{prepare}@(T);
Collect votes from all the nodes involved in T;

//Write phase
if all votes are "commit":
    @\textbf{commit}@(T);
else
    @\textbf{abort}@(T);
\end{lstlisting}
    \caption{Coordinator process code in the template protocol.}
    \label{alg:coord_template}
    \vspace{-1mm}
\end{figure}

%    Run execution phase to get read set R and write set W -- 
%        for each data item d in R, record d's sequence number

\begin{figure}[t!]
\begin{lstlisting}[style=lststyle, frame=tlrb, escapechar=@]
Upon @\textbf{procedure\_x}@(D) from C:
    result = @\textbf{procedure\_x\_handler}@(D);
    Send result to C;
\end{lstlisting}
\caption{Participant process code in the template protocol.}
\label{alg:proc_template}
\vspace{-1mm}
\end{figure}

%\subsection{Strong consistency}

%The consistency level for transactional storage systems describes the accepted behaviour of concurrently executed transactions (i.e., clients start executing transactions concurrently and they may be processed by multiple processes in parallel). A strong consistency level is highly desirable because it helps developers easily reason about and achieve the correctness properties of their application. The most popular consistency level for transactional storage systems is \emph{serializability}, which prescribes that committed transactions appear to have executed serially, one after the other. Formally:

%\begin{definition}[Serializability]
%An implementation of a PDTS satisfies \emph{serializability} if a history that is %equivalent to a legal serial history can be derived from every execution it produces.
%\end{definition}

\subsection{Multicore scalability}

\myparagraph{Disjoint-Access Parallelism} Multiprocessor multicore designs allow hundreds of cores to be placed on a single node, making multicore scalability highly desirable. In order to achieve multicore scalability, all sources of contention among cores must be eliminated. One of the most highly contended resource among cores is the memory; cache coherence protocols utilized by such architectures imply that accessing memory that is also modified by other cores is expensive~\cite{clements13scalablecommutativityrule, boyd2014multiprocessorbottlenecks,ben2017analyzing}. 
%Shared-memory multiprocessor multicore architectures commonly utilize a cache coherence protocol to keep the memory caches consistent. While reading any data and writing data that has been cached exclusively by a core is scalable (i.e., can be done without interference from the other cores), writing a shared cache line is not scalable since updates to shared cached data are serialized by the coherence protocol~\cite{clements13scalablecommutativityrule, boyd2014multiprocessorbottlenecks}.
Moreover, the scalability dramatically degrades when the two cores contending on the same cacheline pertain to different processors (NUMA domains).

While achieving perfect multicore scalability may be impossible for transactional storage systems, since data contention is inherent to many transactional workloads, a couple properties borrowed from the concurrent objects and software transactional memory literature can at least guarantee multicore scalability when processing transactions that do not conflict.

The first property, \emph{disjoint-access parallelism}, was originally introduced to describe the degree of parallelism of implementations of shared memory primitives~\cite{israeli94dap}, and, intuitively, it means that processes execute shared memory primitives on disjoint sets of memory words in parallel, without interfering with each other. The property was later adopted by software transactional memory works to describe implementations where transactions which are unrelated at the high-level, i.e. they access disjoint sets of data items, cannot simultaneously access the same low-level shared memory locations~\cite{attiya2011inherent, peluso2015disjoint}. Multiple versions of disjoint-access parallelism have been circulating in the literature. Our impossibility results consider a relatively strict form of \DAP{}, and holds for any definition that considers more conflicts. %the strongest form and might not hold for the weaker variants.

\Naama{Might be good to contrast it with other forms of DAP and explain what we mean by `strict' (i.e. does it capture a lot of conflicts or few conflicts?)}

\begin{definition}[Strict disjoint-access parallelism]
An implementation of a PDTS satisfies \emph{strict disjoint-access-parallelism} if 
two steps associated with distinct transactions can contend on the same base object only if the transactions' data sets intersect.
%it only produces executions where two steps associated with two distinct transactions contend on the same base object only if the transactions' data sets intersect. %\Naama{define contend}
\end{definition}

\myparagraph{Invisible Reads.} The second property, \emph{invisible reads}, tries to capture the intuition that transactions' read operations should not require any shared memory writes. This property greatly benefits workloads with read hotspots, by dramatically reducing cache coherence traffic.
There are two variants of this property that are common in the literature. The first, which we call \emph{weak invisible reads}, only requires invisible reads at the granularity of transactions. That is, if a transaction is read-only (i.e., its write set is empty), then it may not make any changes to the shared memory. This property has been often used in the theoretical transactions literature~\cite{attiya2011inherent,others}, as it captures a basic requirement for avoiding excessive hotspots, and is easy to define formally. 

\begin{definition}[Weak Invisible Reads]
An implementation of a PDTS satisfies \emph{weak invisible reads} if it only produces executions where every transaction with an empty write set does not execute any non-trivial primitives.
\end{definition}

However, the weak invisible reads property can be somewhat unsatisfying, as it says nothing about the number of shared memory writes a transaction may execute even once it has a since item in its write set. That is, it allows transactions to make shared memory modifications for their read sets as well. In the systems literature when developing systems that decrease coherence traffic, the weak invisible reads property is often not enough. Indeed, many papers that refer to invisible reads in the systems literature~\cite{blah, blah} require that no read operation in the transaction be the cause of shared memory modifications. This is a stricter property, which we call \emph{strong invisible reads}. While this property has been referred to often in the literature, to the best of our knowledge it has never been formally defined until now. The difficulty is in formally map low-level shared memory operations to high-level transaction operations that `caused' them. To get around this challenge, we instead require that, regardless of their read sets, two transactions with identical write sets always produce the same shared memory writes.

%We consider two variants of this property. Our impossibility results hold only for the stronger variant. \Naama{the previous sentence makes our results sound weak. I think we could rephrase this to emphasize the strong version first, how it's been referenced by systems papers in the literature but never defined, how important it is, etc. Then afterwards mention the weaker version and say that interestingly, we show that the weaker one is much easier to achieve... or something like that.} The \emph{strong invisible reads} property requires that no read operation writes to shared memory, while the \emph{weak invisible reads} property requires this to be true only for the read operations of \emph{read-only} transactions, i.e., transactions with an empty write set. The definition of weak invisible reads has appeared in the literature before~\cite{attiya2011inherent}, and is formally as follows.



%The notion of strong invisible reads has only appeared in the literature informally. Its definition is somewhat more complicated than the weaker variant, since there is no clear mapping between the non-trivial primitives that were executed and a transaction's operations. Instead, intuitively, we require that, regardless of their read sets, two transactions with identical write sets always produce the same shared memory writes.

\begin{definition} [Strong Invisible Reads]
Consider execution $E$ and any two transactions $T_1$ and $T_2$ such that the write sets of $T_1$ and $T_2$ are the same. Let $E_1$ be the continuation of $E$ in which $T_1$ executes solo starting from the state immediately after $E$, and $E_2$ be the continuation of $E$ in which $T_2$ executes solo. An implementation of a PDTS satisfies the \emph{strong invisible reads} property if it satsifies weak invisible reads and additionally, for any execution $E$ it can produce, $E_1$ and $E_2$ constructed as described above, contain the same non-trivial primitives.
\end{definition}
%\Naama{Modified the definition to account for concurrency. Should make sure it makes sense. We might want to also require that to have strong invisible reads, you also need to have weak invisible reads. I'm not sure that's implied from the current definition.}

\Naama{Might want to add a blurb about the subtleties of the definition, so that people get that this is one of our contributions.}


Note that the strong invisible reads property complements the \DAP{} property for enhanced multicore scalability. A system that has both allows all transactions that do not conflict, not just the disjoint-access ones, to proceed independently, with no interference. \Naama{Mention that the parallel transactional systems literature has focused on impossibilities between DAP and invisible reads? To emphasize their importance.}

The weak and strong invisible reads properties have been used interchangeably in the literature. Interestingly, however, we show that the weak invisible reads property is much easier to achieve than the strong one; it is possible to construct a serializable parallel distributed transactional system with disjoint-access-parallelism, seamless fault tolerance and one-round-trip commmitment (defined in Section~\ref{sec:distributedProperties}), and \emph{weak} invisible reads, but it is impossible to do the same with the strong version of the property.

\subsection{Multi-Node Scalability}\label{sec:distributedProperties}

\myparagraph{Seamless fault tolerance}
High availability is critical for transactional storage systems as many of their applications expect their data to be always accessible. To increase their availability, storage systems create multiple copies of the data and store them at at least $f+1$ distinct nodes in order to tolerate $f$ simultaneous node failures, where $f$ is a configuration parameter. Some systems use more nodes (e.g. $2f+1$) to allow communication with a quorum that is just a subset of the nodes, thus avoiding a dependence on the slowest node.
%, where a configuration establishes the system's membership. 

However, in most replication schemes proposed in the literature, there is some node that all transactions wait on. In $f+1$ schemes, all nodes act in this role; each client must hear from all nodes to ensure its transaction commits. In others, a \emph{leader} is utilized to easily serialize transactions. These approaches inherently require increased latency due to reconfiguration for the failures of certain nodes (e.g. if the leader fails).
%In most of the replication schemes proposed in the literature, at least one node is common to \emph{all} write quorums used to replicate transactions. Schemes that utilize $f+1$ nodes per configuration require all transactions to be replicated on all $f+1$ nodes. This ensures that the system holds on to the data despite up to $f$ simultaneous node failures. To restore the availability of the system, a reconfiguration protocol is used whenever a node fails. Existing schemes that utilize $2f+1$ nodes per configuration commonly use a primary/leader to establish the order of the operations. Whenever the leader fails, a leader change mechanism is used.

%The two approaches have two disadvantages. First, failures of certain nodes may have a negative impact on all clients -- in the first approach, \emph{any} node failure causes the system to be unavailable until the reconfiguration finishes, and in the second approach, if the leader fails, transactions cannot be processed until the leader change finishes. Second, transaction processing requires communication with certain nodes -- the first approach requires waiting for replies from all $f+1$ nodes, while the second requires waiting for reply from the leader --, which can be expensive if the respective nodes are slow or situated in a different geographical location.

Recently, a few proposals introduced replication schemes for transactional systems that utilize $2f+1$ nodes to tolerate $f$ node failures and do not require a leader~\cite{zhang18tapir, szekeres2020meerkat, mu16janus, kraska13mdcc}. Similar to Fast Paxos~\cite{lamport06fastpaxos}, these schemes employ a \emph{fast path} that requires communication with \emph{any} subset of $q$ (usually $q > f$) nodes in order to process all transactions that do not concurrently conflict with any other transaction. This allows them to \emph{seamlessly} tolerate up to $n-q$ simultaneous node failures when using the interactive transactional model and only affect transactions that were being executed by the failed node when using the stored procedure transactional model.
We formalize this notion, which to the best of our knowledge has so far only been used intuitively in the literature.

%\begin{definition} [q-flexibility]
%An implementation of a PDTS provides \emph{q-flexibility} if a transaction can \emph{terminate} after it communicated with any up to $q$ nodes.
%\end{definition}

\begin{definition}[$f$-seamless fault tolerance]
%Consider an execution $E$ of a PDTS implementation $A$, such that no node fails in $E$. For any transaction $T$ in $E$, let $R_T$ be the number of communication steps in $E|T$. 
%An implementation of a PDTS satisfies f\emph{-seamless fault tolerance} if for any execution $E'$ such that $E'$ is identical to $E$ except that up to $f$ nodes fail (i.e., their steps do not appear in $E'$ after some bounded prefix), the number of round trips in $E'|T$ is $R_T$.

%An implementation of a PDTS satisfies f\emph{-seamless fault tolerance} if for any failure-free execution $E$ it produces there exists an execution $E'$ such that $E'$ is identical to $E$ except that $f$ nodes failed (i.e., their steps do not appear in $E'$ after some bounded prefix) at the beginning of the execution.

An implementation of a PDTS satisfies f\emph{-seamless fault tolerance} if for any failure-free execution $E$ it produces, for every execution $E'$ also producible by the system such that (1) there are up to $f$ node failures in $E'$, (2) $E'$ and $E$ have the same set of transactions and transaction conflicts, the depth of each transaction is the same in both executions.
%terminates in the same number of  and  is identical to $E$ except that $f$ nodes failed (i.e., their steps do not appear in $E'$ after some bounded prefix) at the beginning of the execution.
%\Naama{Change it so that you are seamless only if your owner doesn't crash.}
\Naama{I think we only defined depth of a step, not a transaction. Also, we need to remind people what depth means intuitively, probably in a brief paragraph discussing the meaning of the definition after the definition itself.}
\end{definition}

%\Naama{Should define execution projections $E|T$ in the model, so we can shorten the definition a bit. Also, did we define the number of round trips in an execution?}

%\aaasz{is that definition sufficient?}

%\aaasz{TODO: do we need smth more formal, like the if the system can produce an execution where n-q transactions terminated after they communicated with distinct subsets of q nodes?}

%\Naama{I think we should rename q-flexibility to seamless fault tolerance. Also, the current definition is not seamless because it doesn't talk about how long it takes to terminate.}

\myparagraph{Low commitment latency}
Transactional systems all strive to provide as low latencies as possible. For distributed transactional systems, the cost of network communication accounts for a large fraction of the end-to-end latency of transactions, especially when communication needs to happen between different data centers. Therefore, it is important for distributed transactional systems to reduce the number of message delays (the time it takes for a message to be delivered) required to process transactions. In particular, today's transactional storage systems shoot for committing transactions in a \emph{single round-trip} in the absence of failures and conflicts~\cite{kraska13mdcc, zhang18tapir, szekeres2020meerkat}. ``One round-trip commitment'' has been loosely used to characterize the commitment latency of these protocols and has never been formalized. Here, we give a formal definition of this property.

Intuitively, the commitment process for a transaction starts with ensuring that enough participant processes (shards/replicas) have committed to accepting the transaction. This commitment comes in the form of state modifications (changes to concurrency control metadata) that prevent subsequent correctness violations. To formally identify messages whose handlers' execution can result in \emph{commitment-related state modifications}, we introduce the definition of a \emph{non-trivial message}.

\begin{figure*}[ht!]
    \centering
    \includegraphics[scale=0.23]{figures/trivial_message.pdf}
    \caption{. }
    \label{fig:trivial_message}
    \vspace{-1mm}
\end{figure*}

%However, it is not clear what is meant by ``one round-trip commitment''; when does the ``commitment'' begin?If we consider it to begin from when the client invokes the transaction, even these solutions that claim to achieve ``one round-trip commitment'' would not satisfy such a definition --some do not count the initial message the client sends to the node meant to execute the transaction~\cite{kraska13mdcc}, others do not count the round-trips required for the client to read the data from an arbitrary number of partitions during the execution phase~\cite{zhang18tapir}. We thus introduce a definition that captures the intuition that the commitment phase in all these systems begins once the transaction processing mechanism visibly changes the state of the system, i.e., in a way that can influence other transactions.


%\textbf{Non-trivial message.} We define a \emph{non-trivial message} to be a message whose processing requires at least one non-trivial primitive operation.
%
%Consider a \emph{receive} event of message $m$ in some projection $E|\{p, T\}$. If any step between this receive event and the next receive event in this same projection -- if there is any, if not, we consider all the subsequent steps -- is a non-trivial primitive operation, then $m$ is a \emph{non-trivial message}.

\begin{definition}[Non-trivial message]

Consider a \emph{receive} event of message $m$, $recv(m)$, in some projection $E|\{p, T\}$, such that $recv(m)$ is the last step of $T$ in $E$. Let $\sigma$ be the complete sequence of receive and send events of other transactions that appear after $recv(m)$ in $E$. Let $\pi$ be the prefix of $E$ up, and including, to $recv(m)$. Let $E'$ be an execution with prefix $\pi$, which,  additionally, contains as many steps as possible in the projection $E|\{p, T\}$ (up to the next receive event in that projection), but still reflects $\sigma$. If $E'$ is producible by the system then we say that message $m$ is \emph{trivial} in $E$. A message $m$ is \emph{non-trivial} if there exists an $E$ such that $m$ is not trivial in $E$.

%Let $\sigma$ be the sequence of steps between this receive event and the next receive event in the same projection -- if there is any, if not, we consider all the subsequent steps (intuitively, $\sigma$ is the execution of the handler of $m$). If, after the last step of $\sigma$, there is no step associated with $T$ in $E$ then we can determine if $m$ is \emph{trivial} as follows. 
%Let $E'$ be $E$ from which we first remove all steps that are not \emph{send} after the last step in $\sigma$, then we remove all steps in $\sigma$. If $E'$ is a prefix and a subsequence of an execution producible by the system, then we say message $m$ is trivial in $E$.
\end{definition}

We define the depth of a transaction in an execution to be the number of message delays it takes from when the first non-trivial message was received in the execution of the transaction before the execution of the response step for that transaction.

\begin{definition}[Depth of a transaction]
Consider some projection $P = E|T$, the response step $r$ of $T$ in $P$, and the first receive step in $P$ of a non-trivial message, $recv$. The depth of transaction $T$ is the depth of $r$ in execution $E'$ being a suffix of $P$ starting from $recv$.
\end{definition}

%We are interested in the time it takes for a transaction to be committed in failure-free executions in which there is no concurrent conflicting transaction.
%To measure time despite asynchrony, we consider the number of \emph{message round trips} it takes from when the initiating client sends its first non-trivial message until that client knows the result of the transaction. 
%\Naama{Need  to define "non-trivial message" and justify why we only start counting there.}
%That is, we do not count any memory accesses (to private or shared memory) by processes, and instead only count communication between nodes and between the client and nodes. This choice is motivated by real systems, in which communication on the network is significantly slower than within a single node.
%To allow for algorithms in which the client optimistically computes the result of its transaction locally and then later validates it with the server nodes, we only count round trips starting with the first non-trivial message.

\begin{definition}[One round-trip commitment]
An implementation of a PDTS satisfies \emph{one round-trip commit} if, for every failure-free execution $E$ that it can produce and every transaction $T$ with response $r$ in $E$ that did not execute concurrently with any conflicting transaction, the depth of $T$ is at most 1.
%\Naama{Under the assumption that reads are atomic (we are not interested in how they are made atomic)}
%\Naama{Alternatively: define round trips from the time you know what your data set is.}
%\Naama{This definition doesn't actually use non-trivial messages.}
\end{definition}

\aaasz{TODO: discussion about example protocols that satisfy our definition of one-round trip commitment and show why (what are the non-trivial messages, etc.), and which other class of protocols cannot without additional assumptions (e.g., 2PL)}


%Intuition: for invisible reads, you need to first lock all the write set before validating the read set. This is a pattern seen in a few single-node transactional memories (e.g. Silo).
%Is that true? Can we formalize this requirement?

%If the above is true, does this mean that we need more than one round trip in a distributed setting? I.e. do we need a separate round trip for write-locking and read-verifying? To answer this question, look at counter example sent in Slack. Do we need flexible quorums for that? 

%Maybe parallel dag will help with formalizing dependencies.

%Think of concurrent objects for formal definitions.

%\Naama{Notes and thoughts on definitions:

%two definitions of invisible reads -- one requiring any read operation to be invisible, and the other only requiring read-only transactions to be invisible. The first is stricter, and therefore easier to prove impossibility about. Currently, we only have a lead for showing the first is impossible with DAP, 1-round-trip, and flexible quorums.

%\cite{peluso2015disjoint} defines the first, stricter version. \cite{attiya2011inherent} defines the second. However, I am not very happy with the definition of invisible reads in \cite{peluso2015disjoint}. It refers to read and write operations inside a transaction, and says that a read operation is invisible if it doesn't execute any non-trivial primitive steps. However, it is unclear to me how they define the mapping between a read operation and the primitives that were associated with it. It seems a bit difficult to me, because it's conceivable to think that the primitive steps might be   `mixed', for example, one step is executed to help apply several high-level read/write operations at once. In that case, which operation is that primitive step associated with? This paper seems to assume that a transaction's steps can be partitioned into those belonging to specific high-level operations.

%Another way to potentially define the stricter notion of invisible reads is using the steps executed by the entire transaction, as follows (or something along these lines):

%\begin{definition}
%A system satisfies \emph{invisible reads} if, for any two transactions $T_1$ and $T_2$ whose write sets are the same, the non-trivial primitive steps executed by $T_1$ are the same as the non-trivial primitive steps executed by $T_2$.
%\end{definition}

%The idea is that differences in read sets doesn't allow a difference in the primitive writes that the transactions execute. The above definition doesn't quite work because we need to qualify this by saying they start from the same state, experience the same schedule, etc... Need to think of how to phrase it exactly.

%If we do manage to define something like this, I think it would give us the property that we want. Maybe we'll have to add a requirement that a read-only transaction doesn't execute non-trivial primitives. Then I think the stricter version is implied by requiring that the read-set doesn't affect the non-trivial primitives, like the definition above.


==> sections/todos.tex <==
\begin{itemize}
    \item (FIXED) define projections in model
    \item mention what "desirable properties" is
    \item (FIXED) find definition for communication step (and put in model)
    \item (FIXED) finish one-round-trip commitment definition
    \item (FIXED) Change `round trips' to `communication steps' in relevant parts of the paper
    \item (DONE) go over intro, add more details (Naama)
    \item write conclusion
    \item related work
    \item (FIXED) fix text in 3.4 (Adriana)
    \item (DONE) go over text in 3.3 (Naama)
    \item go over possibilities (Adriana)
        - carefully look at sacrificing DAP section
        - atomic read description
    \item (DONE) make figures for proof be next to each other
    \item Read over entire paper
    \item ABSTRACT (totally forgot, lol; me too lol)
\end{itemize}
